AscendKernelGen: A Systematic Study of LLM-Based Kernel Generation for Neural Processing Units

To meet the ever-increasing demand for computational efficiency, Neural Processing Units (NPUs) have become critical in modern AI infrastructure. However, unlocking their full potential requires developing high-performance compute kernels using vendor-specific Domain-Specific Languages (DSLs), a task that demands deep hardware expertise and is labor-intensive. While Large Language Models (LLMs) have shown promise in general code generation, they struggle with the strict constraints and scarcity of training data in the NPU domain. Our preliminary study reveals that state-of-the-art general-purpose LLMs fail to generate functional complex kernels for Ascend NPUs, yielding a near-zero success rate. To address these challenges, we propose AscendKernelGen, a generation-evaluation integrated framework for NPU kernel development. We introduce Ascend-CoT, a high-quality dataset incorporating chain-of-thought reasoning derived from real-world kernel implementations, and KernelGen-LM, a domain-adaptive model trained via supervised fine-tuning and reinforcement learning with execution feedback. Furthermore, we design NPUKernelBench, a comprehensive benchmark for assessing compilation, correctness, and performance across varying complexity levels. Experimental results demonstrate that our approach significantly bridges the gap between general LLMs and hardware-specific coding. Specifically, the compilation success rate on complex Level-2 kernels improves from 0% to 95.5% (Pass@10), while functional correctness achieves 64.3% compared to the baseline's complete failure. These results highlight the critical role of domain-specific reasoning and rigorous evaluation in automating accelerator-aware code generation. AscendKernGen is available at https://huggingface.co/AscendKernelGen and https://github.com/weich97/NPUKernelBench.

==> tables/kernel-host-decompos.tex <==
\begin{table}[t]
\begin{tcolorbox}[
sharp corners,
      colframe=refgreen,
      colback=refgreen!5,
      colbacktitle=refgreen!15,
      coltitle=refgreen,
      boxrule=0.4pt,
      title={\textbf{Host-Kernel Decomposition}},
      fonttitle=\bfseries\small,
      top=-10pt, bottom=0pt, left=1pt, right=1pt
]
\begin{tabular}{p{0.48\textwidth} p{0.48\textwidth}}
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize]
# Before decomposing
.../{op_name}/answer/
+-- 0/
    |-- op_host/
    |   |-- add_custom.h
    |   `-- add_custom.cpp
    `-- op_kernel/
        |-- add_custom.h
        `-- add_custom.cpp
\end{lstlisting}
&
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize]
# After decomposing
.../{op_name}/answer/
+-- 0/
|   +-- ... (Original backup)
+-- 1/
|   +-- op_host/ (<- The Host code of scenario 1.)
|   |   +-- add_custom.h
|   |   `-- add_custom.cpp
|   +-- op_kernel/
|   |   +-- add_custom.h
|   |   `-- add_custom.cpp
|   `-- tiling_key.json
`-- 2/
    +-- op_host/ (<- The Host code of scenario 2.)
    |   +-- add_custom.h
    |   `-- add_custom.cpp
    +-- op_kernel/
    |   +-- add_custom.h
    |   `-- add_custom.cpp
    `-- tiling_key.json
\end{lstlisting}
\end{tabular}
\end{tcolorbox}
\caption{The kernel code structure before and after decoupling. }
\label{tab:kernel_host_decompos}
\end{table}

==> tables/kernel_example.tex <==
\begin{wraptable}{r}{0.54\textwidth}
\vspace{-10pt}
\centering
\begin{tcolorbox}[
    rounded corners,
    arc=3pt,
    enhanced,
    width=0.54\textwidth,
    colframe=codegreen, % <----- CHANGED
    colback=white,
    title=\textbf{An example of Kernel Code},
    fonttitle=\bfseries\small,
    boxrule=0.6pt,
    left=2pt,
    right=2pt,
    top=0pt,
    bottom=1pt
  ]
  
\begin{tcolorbox}[
      sharp corners,
      colframe=refgreen,
      colback=refgreen!5,
      colbacktitle=refgreen!15,
      coltitle=refgreen,
      boxrule=0.4pt,
      title={\textbf{Host}},
      fonttitle=\bfseries\small,
      left=0.5pt,
      right=0.5pt,
      top=-5pt,
      bottom=-5pt
    ]
\begin{lstlisting}[style=mystyle, frame=none,framerule=0pt, language=Python]
namespace optiling {
static ge::graphStatus TilingFunc(gert::TilingContext *context)
{ // Initialize tiling data structures and parameter configurations
    TilingData tiling;
    return ge::GRAPH_SUCCESS;
}
} // namespace optiling
namespace ops {
class AddCustom : public OpDef {
public:
    explicit AddCustom(const char *name) : OpDef(name)
    {// Define operator input/output types and computation configuration
    }
};
OP_ADD(AddCustom);
} // namespace ops
\end{lstlisting}
\end{tcolorbox}
\begin{tcolorbox}[
      sharp corners,
      colframe=refgreen,
      colback=refgreen!5,
      colbacktitle=refgreen!15,
      coltitle=refgreen,
      boxrule=0.4pt,
      title={\textbf{Kernel}},
      fonttitle=\bfseries\small,
      left=0.5pt,
      right=0.5pt,
      top=-5pt,
      bottom=-5pt
    ]
\begin{lstlisting}[style=mystyle, frame=none,framerule=0pt, language=Python]
class KernelAdd {
public:
    __aicore__ inline void Init(GM_ADDR x, GM_ADDR y, GM_ADDR z, uint32_t totalLength, uint32_t tileNum) { // Initialize global buffers and queues
    }
    __aicore__ inline void Process() {
        for (int32_t i = 0; i < loopCount; i++) {
            CopyIn(i);
            Compute(i);
            CopyOut(i);
        }
    }
private:
    __aicore__ inline void CopyIn(int32_t progress) {
    // Copy xGm and yGm to local tensors via inQueue
    }
    __aicore__ inline void Compute(int32_t progress) {
    // Dequeue xLocal, yLocal; perform Add; enqueue zLocal
        LocalTensor xLocal = inQueueX.DeQue<DTYPE_X>();
        LocalTensor yLocal = inQueueY.DeQue<DTYPE_Y>();
        LocalTensor zLocal = outQueueZ.AllocTensor<DTYPE_Z>();
        Add(zLocal, xLocal, yLocal, tileLength);
    }
    __aicore__ inline void CopyOut(int32_t progress) {
    // Copy zLocal back to zGm
    }
};
extern "C" __global__ __aicore__ void add_custom(GM_ADDR x, GM_ADDR y, GM_ADDR z) {
    KernelAdd op;
    op.Init(x, y, zzh);
    op.Process();
}
\end{lstlisting}
\end{tcolorbox}
\end{tcolorbox}
\vspace{-15pt}
\captionof{table}{AscendC kernel for vector addition.}
\label{tab:kernel_example}
\vspace{-30pt}
\end{wraptable}


==> tables/single_file_qa_prompt.tex <==
\begin{wraptable}{l}{0.5\textwidth}
\vspace{-20pt}
\centering
\begin{tcolorbox}[
    sharp corners,
      colframe=reforange,
      colback=reforange!5,
      colbacktitle=reforange!15,
      coltitle=reforange,
      boxrule=0.4pt,
      title={\textbf{Prompt for generating question}},
      fonttitle=\bfseries\small,
      left=0.5pt,
      right=0.5pt,
      top=0.5pt,
      bottom=0.5pt
]
{\small
You are an expert in AscendC programming for the Huawei Ascend processor. Based on the provided answer code, please generate a corresponding request for that code.

\textbf{Background:} 

I maintain an AscendC operator repository that contains many operators, and each operator consists of multiple code files. I am constructing a dataset to train an LLM that can assist in writing AscendC operators. Each file within an operator will serve as a single training sample. I already have the answer code for each sample, but I still need to generate the corresponding request. After I provide you with a piece of answer code, your task is to analyze the code, understand and summarize its purpose, and then generate a request such that the provided code naturally serves as a correct response to that request. The request should be high-level and concise rather than overly detailed.

Please output the request in the following format:

\verb|<request>REQUEST_TEXT</request>| 

Note: Output only the final request—no reasoning process.

\textbf{Requirements:}

1. The request must capture the core functionality and purpose of the code.

2. The request should be clear and concise, avoiding unnecessary complexity.

The answer code is provided below:

[ ... Kernel code ... ]

}
\end{tcolorbox}
% \begin{tcolorbox}[
%     sharp corners,
%       colframe=reforange,
%       colback=reforange!5,
%       colbacktitle=reforange!15,
%       coltitle=reforange,
%       boxrule=0.4pt,
%       title={\textbf{Generated question samples}},
%       fonttitle=\bfseries\small,
%       left=0.5pt,
%       right=0.5pt,
%       top=0.5pt,
%       bottom=0.5pt
% ]
% {\small
% <request> Please create an interface header file for the Sigmoid operator that includes the required header references, uses the AscendC namespace, and provides a deprecation notice pointing to the new sigmoid.h file. </request>

% <request> Please implement an AscendC operator header file that defines the computation interface for the Swish activation function. The activation is defined as swish$(x) = x / (1 + e^{(-βx)})$, and it should support both half and float data types. </request>
% }
% \end{tcolorbox}
\vspace{-15pt}
\captionof{table}{Prompt for generating question.}
\label{tab:prompt_single_file_qa}
\vspace{-100pt}
\end{wraptable}


